Bayesian inference under model misspecification using transport-Lagrangian distances: an application to seismic inversion

Model misspecification constitutes a major obstacle to reliable inference in many inverse problems. Inverse problems in seismology, for example, are particularly affected by misspecification of wave propagation velocities. In this paper, we focus on a specific seismic inverse problem - full-waveform moment tensor inversion - and develop a Bayesian framework that seeks robustness to velocity misspecification. A novel element of our framework is the use of transport-Lagrangian (TL) distances between observed and model predicted waveforms to specify a loss function, and the use of this loss to define a generalized belief update via a Gibbs posterior. The TL distance naturally disregards certain features of the data that are more sensitive to model misspecification, and therefore produces less biased or dispersed posterior distributions in this setting. To make the latter notion precise, we use several diagnostics to assess the quality of inference and uncertainty quantification, i.e., continuous rank probability scores and rank histograms. We interpret these diagnostics in the Bayesian setting and compare the results to those obtained using more typical Gaussian noise models and squared-error loss, under various scenarios of misspecification. Finally, we discuss potential generalizability of the proposed framework to a broader class of inverse problems affected by model misspecification.

==> Section2_LitRew/FWI.tex <==
\subsection{Full-waveform seismic inversion} \label{sec:LitRew:FWI}
\todo{This is a section I'd like to shorten dramatically. I think the main goal could be to introduce the moment tensor inversion problem, but that actually comes already in Section 4. So here what do we want to do? What does the reader *really* need to know or be aware, in order to understand either the details or context of what comes next?}
In this subsection we present a brief overview of the main approaches to seismic inverse problems (including, but not limited to, moment tensor estimation). The goal is not to provide exhaustive reviews on the topic (which already exist elsewhere), but instead highlight the main challenges that arise in this kind of application and use them as a motivator for our approach.

\subsubsection{Local optimization based approaches} \label{sec:LitRew:localoptim}
Waveform inversion started to become a problem of interest in seismology since the introduction of seismograph networks capable of recording accurate seismic data (both active and passive). The most traditional approach to seismic inversion is non-probabilistic i.e., the model parameters are recovered by optimizing a misfit function defined over observed $y(t)$ and model-predicted $u(t)$ waveforms \cite{virieux2009overview}:
\begin{equation}
	\mathcal{M}(\theta) = \mathcal{M}({y(t),u}(\theta,t)), \label{eqn:misfit}
\end{equation}
where $\theta$ indicates any subset of the parameters of interest to be recovered (velocity field, earthquake location, moment tensor, density of the media etc.).
However, given the complexity of the forward model and ill-posedness of the inverse problem, the minimization of $\mathcal{M}$ is often performed locally, meaning the gradient of the objective function (\ref{eqn:misfit}) is taken locally with respect to perturbations $\Delta \theta$ of an initial model configuration $u(\theta_0)$ \cite{virieux2009overview}:
\begin{equation}
	\mathcal{M}(\theta) = \mathcal{M}(\theta_0 + \Delta \theta). \label{eqn:misfitpert}
\end{equation}
%
Typically, misfit functions are chosen to be norms, with the least-squares ($L^2$) norm being the most popular choice \cite{Tarantola1986}. A number of techniques (Newton, Truncated-Newton \cite{Virieux2013},Gauss-Newton, gradient or steepest descent) are used to solve, under various assumptions, the optimization problem. The ill-posedness of the seismic inverse problem and associated non-convexity of $\mathcal{M}(\theta)$ has motivated further attempts to constrain the number of possible solutions beyond the perturbation/linearization methods just discussed. Regularization of the objective function such as Tikhonov regularizers  or wighting or inverse covariance matrices are part of the classic repertoire \cite{Virieux2013b,Diaz2012,Leeuwen2013}. Recent advances in compressive sensing and the associated idea of randomized data sampling have also motivated approaches to full‐waveform inversion that look for for sparse solutions \cite{Hermann2012}. \\

 Alternative measures of misfit have also been proposed such as the $L^1$ norm, secant ($sech$) and mixed $L^1$-$L^2$ norms (Huber penalty) \cite{Tarantola1990}, as well as optimal transport based misfit functions \cite{Viriuex2016,Chen2018,Virieux2016c,Warner2013}. In \cite{Becker2015} the authors proposed a general robust algorithmic framework to account for different types of misfit functions and regularization terms. The algorithm relies on quasi-Newton Hessian approximation methods to minimize the misfit function and proximal gradient methods to minimize the regularizing terms. \\


Gradient-free methods have also been adopted. In the context of downhole micro-seismic moment tensor inversion \cite{Toksoz2011}, a grid-search is performed over plausible event locations and velocity models. The best fitting solution, in a least squares sense, is then identified.  In a similar fashion, a large body of literature exists on how to constrain the number of feasible solutions by estimating source-receiver travel times and rejecting solutions that are not compatible  (ray-tracing techniques) \cite{shearer2009introduction}.  \\ 

Solutions of the problem both in the time and frequency domain have also been attempted \cite{Demanet2014b,Virieux2009}. The advantage of using one method over the other depends on several factors such as the type of data available (high/low frequency, noise level etc.) as well as what kind of information is recovered in the inversion. In \cite{Vavrycuk2012} the moment tensor inversion is performed through a two step procedure involving an inversion both in the time and frequency domains, exploiting the linearity of $\mathbf{u}(t)$ in $\mathbf{m}$ when the velocity model and source location are fixed. \\

Multiscale or multifidelity approaches have also been adopted in the spirit of mitigating the computational complexity and ill-posedness of the problem \cite{Plessix2009,Bunks1995}. Given the recent advances in computational power, some attempts to 3D full-waveform inversion have also been made \cite{Plessix2009,Virieux2016c}.  \\


The main bottleneck in the successfulness of these approaches is the accuracy of the starting model and assumptions underlying the various simplifications (e.g., linearization). It is hard to build a valid prior model, especially when it comes to estimating the velocity $\mathbf{V}$. Starting with a highly misspecified model inevitably leads to bad parameter estimates. The problem is even more accentuated by considering only one-point estimates (typical of deterministic inversion), since the amount of uncertainty that surrounds the solution is largely ignored. We argue a Bayesian framework offers a more complete representation of the current state of knowledge and is particularly relevant in a misspecified setting.

\subsubsection{Bayesian formulations}
An extensive amount of work exists around full-waveform inversion performed in a Bayesian framework \cite{Bosch2010,duijndam1988bayesian,gouveia1998bayesian,sen1996bayesian,ray2017low,gunning2007detection}. We recall that a Bayesian framework is such that both the parameters of interest and the observed data are considered as random variables. A prior probability distribution is assigned to the parameters, a statistical model is then defined, which induces a probability distribution over the observed data conditioned on the model parameters value (otherwise known as likelihood function). Given a prior distribution and a likelihood function, the inversion is achieved by characterizing the posterior distribution:
\begin{equation}
	p(\theta| {y(t)})=\frac{p(y(t)|\theta ) \cdot p(\theta)}{p({y(t)})} .\label{Bayes}
\end{equation}
%
As already stated in the introduction, the most common statistical assumption regarding the relation between observations and model predictions is that of additive Gaussian noise (\ref{eqn:Gaussian_noise_additive_sect1}).
As for the prior distribution, its choice largely depend on the information available to analyst prior to the inversion. A central aspect of Bayesian computation in seismic inversion is the computational cost associated to evaluating the posterior distribution and its marginals. Characterizing the moments of the posterior distribution or calculating the normalization constant $p({y(t)})$ is often impossible analytically and involves high dimensional integrals when performed numerically. For iterative methods, the computation of the forward model at each iteration also poses computational challenges. In \cite{sen1996bayesian, de2017bayesian} a number of sampling approaches have been considered from Markov Chain Monte Carlo (MCMC) to Gibbs sampling and other techniques mutuated from genetic sciences.  An interesting approach to mitigate the dimensionality issue implicit in seismic Bayesian inverse problems is the trans-dimensional Markov Chain Monte Carlo sampler implemented in \cite{ray2017low}. This method represents a way to compromise between  computational cost and modelling accuracy. The cited work relies however on the parameterization of the velocity field through wavelets, which represents itself a simplification of the phenomenon. A similar approach for velocity and density recovery is also implemented in \cite{ray2016frequency} with similar results. \\

Given these challenges, Bayesian approaches to full-waveform inversion have usually required some degree of simplification of the problem to make it tractable. In \cite{Burland2003} the authors propose a Bayesian approach in which the forward model is linearized in the velocity $\mathbf{V}$. The error and the prior distribution are chosen to be Gaussian, which allows the posterior distribution to be derived analytically. The results of this study show that, given a synthetic data-set, although good agreement is found with the correct solution, a signal to noise ratio of 15 (relatively weak noise) introduces high degrees of uncertainty in the solution.  The simplifications introduced are probably partly responsible for these unsatisfactory results. In \cite{BuiThan2013} the authors also linearize the problem, but around the maximum a-posteriori probability estimate (MAP). Despite the simplification, the computational challenge of determining the MAP persists. It involves a non-linear (and possibly non-convex) optimization problem and there is no guarantee that the approximation will be good enough.  Other Bayesian inversion attempts with linearized models can be found in \cite{gunning2007detection, grana2010probabilistic}. An alternative consists in pre-computing the forward model over a grid of possible parameter values \cite{spikes2007probabilistic}. While computationally efficient, this approach poses the question of how  fine the grid over the parameter space has to be and  it can become impractical when performing multi-parameter inversion. 

In \cite{gu2017waveform} the authors attempted a full Bayesian inversion without any simplification of the forward model or linearization around specific solutions. To overcome the computational challenges and increase robustness of the solution, a number of sampling strategies are implemented to exploit conditional linearities and associated Gaussianities in the problem. These include marginal-then-conditional sampling, pre-computing  a library of velocity models and source locations as well as \textit{coarsening} as described in \cite{miller2018robust}. The results achieved through this implementation are satisfactory when the velocity is known and set to a specific value. As soon as uncertainty is introduced in $\mathbf{V}$, the solutions of the problem exhibit a high degree of instability, indicating model misspecification issues. \\

This once again serves as a motivator for adopting different approaches to deal with model misspecification, using moment tensor inversion as a testbed for our methodology. 

==> Section2_LitRew/OT_long.tex <==
\subsection{Optimal transport as misfit measure}
\todo{Again some shortening here. I think the plan here should be to mention past work that uses OT (of various kinds) to build a misfit function in estimation/inference/inverse problems and then get right into the TL distance specifically. It's only on this last point that we need to define things precisely and with all the equations.\\
Also, one thing that strikes me here is that we are already in a setting where we have assumed that the data are "signals" or waveforms, i.e., functions of time. If that is indeed the scope, then let's make it explicit!}

Central to any inverse problem, both in the deterministic and Bayesian framework, is the choice of a misfit function to compare model and predicted data. We have described in the introduction how choosing this metric can play a determining role in performing good inference, especially when dealing with time series. The following discussion  will therefore focus on this specific data-type, except when stated otherwise. \\

The most recurrent choice is the $\ell_2$ norm (least-squares), which is also implicitly obtained by adopting the traditional model that defines observations as model prediction plus Gaussian noise. Being an $\ell_{p}$-norm, the Euclidean distance compares two data vectors element-wise. This represents a limitation when data points are signals (even though discretized), since they inherently exhibit a temporal-spatial structure that cannot be captured by simply comparing them along the time domain. In fact $\ell_p$ norms  ignore the correlation that exists between different points of the signals and can provide rather distorted distance measures.

Some literature exists about possible choices for distance measures between time signals  for a variety of purposes such as pattern recognition, signal classification, detection etc \cite{lauwers2017time}. Some still make  use of the $L^2$-distance, but only on slices of the signals, or after performing a circular shift of the time domain \cite{gharghabi2018ultra}. Other approaches propose counting the number of subsequences of the signals that are similar in an $L^2$ sense \cite{gharghabi2018ultra}. Parameterizations of the signals (i.e., low-rank approximation) have also been proposed such that the comparison is made in this alternative domain rather in the original time or space one \cite{basseville1989distance, chan2008wavelet}. While attractive, these techniques are only relevant to specific  applications and therefore tend to have limited applicability.

\subsubsection{The optimal transport problem}

Recent advances in the domain of optimal transport and its many applications have lead a number of contributions in the field of signal analysis. Optimal transport allows the type of ``horizontal'' comparison of functional data being sought, with some distinctive features compared to the more commonly know dynamic time warping. 

Classical optimal transport (OT) is defined between two probability measures (Kantorovic problem) and solves an assignment/matching problem between the masses at each point of the distributions. All the mass from a measure $a$ must be re-allocated across the points of a measure $b$, satisfying some constraints, at minimal cost. Traditionally the cost function is a distance between the points in the support of the distribution, in which case the solution of the OT problem is referred to as p-Wasserstein distance. In formulas:
\begin{align}
    \mathcal{W}_p(a(x) || b(y)) &= \min_{P_{i,j}} \sum_{i,j} C_{i,j} P_{i,j}; \nonumber \\
    \text{s.t.} \,\,\,\,\, \sum_{j=1}^M P_{i,j} &= a(x_i); \nonumber \\
     \,\,\,\,\,\,\,\,\,\,\,\,\, \sum_{i=1}^N P_{i,j} &= b(y_j); \\
     P_{i,j} &\geq 0; \,\, P \in \mathbb{R}^{N \times M}; \nonumber \\
     C_{i,j} &= |x_i - y_j|^p. \nonumber 
\end{align}
%
The constraints ensure that the transport plan $P \in \mathbb{R}^{N \times M}$ has the two measures as its marginals, while the cost being a $\ell_p$ distance discourages displacements of mass too far apart the original point.
The reason why the value of the objective at optimality can be considered a distance is that the more two measures are different, the more mass will have to be displaced further away across the support from the original location in order to satisfy all the constraints. Displacing to relatively far points between the supports of the two measures increases the overall cost. On the contrary, if the two measures had an equal number of points ($M=N$) and were exactly identical  ($a(x_i)=b(y_i) \,\, \forall i$), then we would have that the total distance is zero. The p-Wasserstein distance possesses the properties of a distance: it is symmetric, respects the triangle inequality  and equals zero only if the the two measures are identical. A distinctive feature of Wasserstein distances v.s. dynamic time warping is that causality is not ensured. This may seem a limitation in its application to signal comparison because of the inherent sequential nature of time signals. However, when dealing with model misspecification this aspect  can actually be beneficial in that inconsistencies in the modeling can produce anticipation or delay in the reproduction of some parts of the observed signal.   \\

 However, a more constraining aspect exists that requires some adaptation for the classical p-Wasserstein distance to be used as a measure to compare time signals. For the OT problem to even have a solution, it is in fact  necessary that the $a$ and $b$ have equal mass i.e., ($\sum_i a(x_i) = \sum_j b(x_j)$) and have non-negative elements. These conditions are naturally satisfied by probability measures, signals however are not measures i.e., they do not sum up to 1 and are not non-negative. A common workaround to this problem is to shift the signal along the ordinate axis to make it positive and then normalize it \cite{Engquist2017,Viriuex2016,thorpe2017transportation}. 
\begin{equation}
	\tilde{a}= \frac{a+ \alpha}{\sum (a +\alpha)}.
\end{equation}
%
Having the signal transformed in such a way also allows a fast, analytical, computation of the Wasserstein distance in 1-D.   
Successful attempts of using the Wasserstein distance in this fashion have been made in the field of waveform inversion too \cite{Engquist2017,Viriuex2016}. Promising results were achieved in these works for velocity inversion. As mentioned in the introduction, the use of OT-based misfit functions has proved to be benficial in terms on non-cenvexity reduction and cycle-skipping effects. \cite{brossier2015velocity,warner2013full}. \\

While computationally convenient, the transformation of the signals that is required appears somewhat artificial and not justified by the physics of the problem. In addition the transformation can distort the signal, smoothing out amplitude vs frequency differences \cite{thorpe2017transportation}.  One approach that avoids this kind of pitfalls is to use the so called transport-Lagrangian (TL) distance, which is a specific instanciation of the Wasserstein distance with the following formulation:
\begin{align}
    TL^{\lambda}_p(a(x) || b(y)) &= \min_{P_{i,j}} \sum_{i,j} C_{i,j} P_{i,j}; \nonumber \\
    \text{s.t.} \,\,\,\,\, \sum_{j=1}^M P_{i,j} &= \frac{1}{N}; \nonumber \\
     \,\,\,\,\,\,\,\,\,\,\,\,\, \sum_{i=1}^N P_{i,j} &= \frac{1}{M}; \label{eqn:TL-dist}\\
     P_{i,j} &\geq 0; \,\, P \in \mathbb{R}^{N \times M}; \nonumber \\
     C^{\lambda}_{i,j} &=  \lambda * |x_i - y_j|^p + |a(x_i) - b(y_j)|^p. \nonumber 
\end{align}
%
This formulation can be interpreted in two different ways:
\begin{enumerate}
    \item optimal transport between two 2-D uniform measures defined on $\{x_i \times a(x_i)\}$ and $\{ y_j \times b(y_j)\}$ i.e., OT between Lebesgue measures raised onto the graphs of $a$ and $b$ $\tilde{a} (x_i \times a(x_i)) = \mathcal{L}(x_i \times a(x_i))$ and $\tilde{b} (y_j \times b(y_j)) = \mathcal{L}(y_j \times b(y_j))$ ;
    \item optimal transport between two (1-D) uniform measures where the cost is defined as $C^{\lambda}(x_i,y_j) = \lambda |x_i - y_j|^p +  |a(x_i) - b(y_j)|^p$;   
\end{enumerate}

This distance is particularly interesting as it avoids unnatural data transformations while still allowing an OT formulation.  In addition, while the Wasserstein distances amounts to solving a linear programming (LP) problem ($N^3$ complexity, with N being the dimension of the signal-vector), for the special case of the TL distance one can adopt more specialized algorithms that solve an assignment problem (i.e., N=M, and P are permutation matrices). The algorithm of our choice is the auction algorithm \cite{bertsekas1981new}, which exhibits a nearly quadratic complexity or average complexity of $N^2 log(N)$  for problems with $N < 1000$ \cite{schwartz1994computational,metivier2019graph} .\\

Rigorous discussion on the applicability of the TL measure as an objective function in deterministic inversion has been conducted in \cite{metivier2019graph}. Particularly the authors have defined a methodology to compute the gradient of a TL misfit and applied it to a seismic imaging problem. Once again improvements in the convexity of the misfit have emerged as the primary effect of the choice of such a distance measure. \\

In this paper we intend to define a strategy for the use of the TL in a Bayesian setting. 



